Toward the Design of Fault-Tolerance- and Peak- Power-Aware Multi-Core Mixed-Criticality Systems

Mixed-Criticality (MC) systems have recently been devised to address the requirements of real-time systems in industrial applications, where the system runs tasks with different criticality levels on a single platform. In some workloads, a high-critically task might overrun and overload the system, or a fault can occur during the execution. However, these systems must be fault-tolerant and guarantee the correct execution of all high-criticality tasks by their deadlines to avoid catastrophic consequences, in any situation. Furthermore, in these MC systems, the peak power consumption of the system may increase, especially in an overload situation and exceed the processor Thermal Design Power (TDP) constraint. This may cause generating heat beyond the cooling capacity, resulting the system stop to avoid excessive heat and halting the processor. In this paper, we propose a technique for dependent dual-criticality tasks in fault-tolerant multi-core MC systems to manage peak power consumption and temperature. The technique develops a tree of possible task mapping and scheduling at design-time to cover all possible scenarios and reduce the low-criticality task drop rate in the high-criticality mode. At run-time, the system exploits the tree to select a proper schedule according to fault occurrences and criticality mode changes. Experimental results show that the average task schedulability is 74.14% on average for the proposed method, while the peak power consumption and maximum temperature are improved by 16.65% and 14.9 C on average, respectively, compared to a recent work. In addition, for a real-life application, our method reduces the peak power and maximum temperature by up to 20.06% and 5 C, respectively, compared to a state-of-the-art approach.

==> Sections/ModelsFinal.tex <==
\section{System Models and Problem Definition}
\label{sec:models}

\subsection{Mixed-Criticality Task Model}
\label{subsec:mixedCriticalityTaskModel}

The MC system is responsible for executing application \textit{A} consisting of multiple dependent periodic tasks. Analogous to~\cite{baruah16,Medina18,Medina181,Ranjbar2020}, the application is modeled as a~directed acyclic graph $\textit{G}_{A}$ ($\textit{V}_{A}, \textit{E}_{A}$) in which each task in the~application is either a HC or a LC task. %\cite{baruah16,Medina17,Medina18,Medina181,Ranjbar19}. 
Each node $\textit{T}_{i}\in\textit{V}_{A}$~represents a task and an edge $\textit{e}_{ij}\in\textit{E}_{A}$ from $\textit{T}_{i}$ to $\textit{T}_{j}$ indicates a dependency between $\textit{T}_{i}$ and $\textit{T}_{j}$. A task is released and ready to be executed if all its predecessor tasks have finished their execution.
We assume preemptive execution for tasks, which means the tasks are interrupted during their execution on a core that mapped on it. 
%Each task in the application is either HC or LC \cite{baruah14, huang15, muller14, huang14, guo14, ali15, narayana16, taherin15, baruah16, socci15, kang14}. %\bnz{\st{, and they have non-preemptive execution which means the tasks are not interrupted during their execution.}}
Each task $\textit{T}_{i}$ is defined as: %$\textit{T}_{i} = (\zeta_{i}, \textit{C}_{i}^{LO}, \textit{C}_{i}^{HI}, \textit{d}_{i}, \textit{P}_{i})$
\begin{align}
	\textit{T}_{i} &= (\zeta_{i}, \textit{C}_{i}^{LO}, \textit{C}_{i}^{HI}, \textit{d}_{i}, \textit{P}_{i})
\end{align}	

%\behnaz{Analogous to~\cite{Medina2018,Baruah2016}, we consider dual-criticality system where each dependent MC task can be either high-critical ($\zeta_i$~=~HC) or low-critical ($\zeta_i$~=~LC)}

Parameter $\zeta_{i}$ denotes levels of criticality for each task (HC or LC). 
Each task has a deadline ($\textit{d}_{i}$), low WCET ($\textit{C}_{i}^{LO}$), and high WCET ($\textit{C}_{i}^{HI}$). 
For each LC task, $\textit{C}_{i}^{LO}$ is equal to $\textit{C}_{i}^{HI}$, and for each HC task, $\textit{C}_{i}^{LO}$ is less than $\textit{C}_{i}^{HI}$.
The communication time between tasks is considered as a part of the predecessor task's execution time. 
All tasks in application \textit{A} have an identical period ($\textit{P}_{i}$), which is equal to the period of the application ($\textit{P}_{A}$)~\cite{salehi16, Ranjbar19}. 
Also, we assumed the deadline and period of the task graph are equal for an application~($\textit{d}_{A} = \textit{P}_{A}$). A deadline $d_i$ is determined for each task in order that all its successors can be scheduled before their deadlines. Hence, the deadlines of tasks that have no successors are equal to the task graph's deadline. 

\behnaz{\textbf{MC system's operational model:} MC systems first start the operation in the LO mode; if the execution time of at least one HC task exceeds its low WCET~($\textit{C}_{i}^{LO}$), the system switches to the HI mode. It stays in this mode until there is no ready HC task in each core's queue~\cite{baruah16,Medina18,Medina181,Ranjbar19}.} % and the remaining HC tasks are executed under $\textit{C}_{i}^{HI}$ .
In the LO mode, the mapping and scheduling algorithms consider the low WCET of tasks while in the HI mode, the algorithm schedules tasks by their high WCETs.


The task graph model is popular for image processing in automotive systems and pedestrian detection~\cite{izosimov10}. System designers assign the criticality level of tasks based on their functionalities. 
However, similar to previous studies in the literature~\cite{baruah16,Medina18}, if an LC task is a predecessor of an HC task, then it is considered as an HC task.
Fig.~\ref{fig: reallife application} shows the task graph of Unmanned Air Vehicle (UAV), which is a real-life MC application task graph~\cite{Medina18}.
This application is composed of eight tasks.
Tasks $\textit{T}_{1}$ to $\textit{T}_{3}$ are HC tasks that are responsible for the avoidance, navigation, and stability of the system.
Failure in the execution of these tasks before their deadline may lead to a system failure, and irreparable damage to the system.
The roles of LC tasks~($\textit{T}_{4}$ to $\textit{T}_{8}$), are recording sensors data, GPS coordination, and video transmissions~\cite{Medina18}.
The system should execute these tasks to improve its QoS; however, the system can skip executing them in harsh situations. Note that, the QoS is defined as the percentage of executed LC tasks in the HI mode to all LC tasks~\cite{li18,Ranjbar2020Fantom} ($QoS= n_L^{succ}/n_L$, where $n_L$ is the number of all LC tasks in a graph and $n_L^{succ}$ is the number of executed LC tasks that, when the system switches to the HI mode and $Finish-time_i\leq d_i \And \zeta_i= LC$). 
\behnaz{Dropping some LC tasks in the HI mode can be used for real-time applications characterized by hard and firm deadlines. % or may have some non-critical tasks. 
The tasks with a hard deadline can be HC tasks, and with firm deadlines %and not-critical 
can be LC tasks. The multimedia tasks are an example of firm deadlines, where skipping a video frame once in a while is better than processing it with a long delay or not processing it completely~\cite{buttazzo11}. }


\begin{figure}[t]
	\includegraphics[width=\linewidth]{imgs/Fig1-PPM.pdf}
	\caption{An example of real-life application task graph (Unmanned Air Vehicle)}
	\label{fig: reallife application}
\end{figure}

\subsection{Fault-Tolerance Model}
\label{subsec:faultTolerantModel}
Transient faults are the most common faults in embedded systems~\cite{guo14,Ranjbar2020Fantom,sahoo2021reliability}. \behnaz{To tolerate transient faults, fault detection and correction mechanisms need to be applied. The detail of these mechanisms is discussed in Appendix A of~\cite{Ranjbar2021}.}%Appendix A.}
%Researchers in~\cite{koren07,siewiorek2017reliable,Bolchini13,Cerrolaza2020} give a comprehensive study in the field of fault detection and correction mechanisms. In general, the key of these mechanisms is using the redundancy, which could be information such as error detection codes, resources such as duplication~\cite{siewiorek2017reliable,koren07}, and analytical, such as learning-based detection approaches~\cite{Iqbal2019}. A comparison of recent mechanisms has been studied recently in~\cite{Thati2018}.}

\behnaz{For embedded safety-critical real-time systems, low-cost, low power, and high accuracy checker should be employed in each core. 
To check whether a fault occurs during the execution of a task, analogous to~\cite{salehi16,Ansari2018,Ranjbar2020Fantom}, an error detection mechanism, %like sanity check~\cite{koren07}, 
is conducted to check the correctness of the task's output at the end of the task's execution. ARGUS~\cite{Meixner2007} is one of the significant checker tools to detect errors, that has all the features and has been used in many recent works~\cite{Cerrolaza2020}. It can be applied to any embedded systems with less than 11\% chip area overhead and also check control flow, dataflow, computation, and memory access separately, at run-time. %ARGUS, which can be applied to any embedded systems with less than 11\% chip area overhead, detects transient and permanent errors. 
Here, the error detection time overhead is considered in the WCET of tasks. Besides, the task re-execution technique is one of the most popular ways to correct transient faults in embedded systems~\cite{Ranjbar2020Fantom, koren07}, which we employed in this article. }%sorin09
We assume that up to~\textit{k} transient faults may occur in one period of the application~\cite{Izosimov08,izosimov10,Salehi2016}. If the system detects a faulty task, it spends some time~($\mu$) to discard the results of the faulty task before re-executing the task. 




\subsection{Power Model}
\label{PowModel}
The total power consumption of a core in an embedded system consists of three major components, Dynamic power~($P_{d}$), static power~($P_{s}$), and frequency-independent power~($P_{ind}$)~\cite{taherin15,Ranjbar19}. 
\answersnd{We consider a pessimistic approach to obtain the dynamic power consumption of HC tasks as well as LC tasks.}
$P_{d}$ is a frequency and workload dependent power which is consumed when a task is run. 
$P_{s}$ is consumed in a core even when the core is in idle mode and no task is run. 
The frequency-independent power is the power used for memory and I/O operations~\cite{taherin15,guo14}. 
The total power is:
\begin{equation}
\label{eq:Power} 
\begin{split}
P(V_i,f_i) &= P_{d} + P_{s} + P_{ind} = \alpha C_{eff}V_i^2f_i + I_{sub}V_{i} + P_{ind}
\end{split}
\end{equation}
where $\alpha$, $I_{sub}$, $C_{eff}$, $f_i$, and $V_i$ are transition rate, sub-threshold leakage current, effective capacitance, core $i$ processing frequency, and core $i$ supply voltage, respectively.




\subsection{Problem Definition}
\label{sec:problemFormulation}

%The MC system is responsible for running application \textit{A} with a set of periodic tasks on a multi-core chip, which is described in \sectionRef{subsec:mixedCriticalityTaskModel}.
%The system might face up to \textit{k} transient faults in one period of the application, and any of the HC tasks overrun their low WCETS.


%As mentioned, the goal of our proposed method is managing the system peak power in both criticality modes ($Cr_L= LO/HI$). Therefore, t
\textit{Deadline Constraint:} Each HC task $\tau_i$, must finish its execution ($ft_i$) correctly before its deadline ($d_i$) in both LO and HI modes. In addition, all LC tasks should finish their execution before their deadlines in the LO mode.
\begin{align}
\forall \tau_i,& ~\zeta_i= HC: ft_i \leq d_i \nonumber \\
\forall \tau_i,& ~\zeta_i= LC \AND Cr_L= LO: ft_i \leq d_i 
\end{align}


%\begin{align}
% &Cr_L= LO\And HI:  &\forall \tau_i \And \zeta_i= HC, ft_i \leq d_i \nonumber \\
% &Cr_L= LO: &\forall \tau_i \And \zeta_i= LC, ft_i \leq d_i 
%\end{align}

\textit{Task Dependability Constraint:} Due to the precedence correlations between tasks, the start time of task $\tau_i$ ($st_i$) must be \behnaz{greater} than the finish time of all its predecessor tasks ($Pred (\tau_i)$).
\begin{align}
\forall \tau_i, \forall j\in Pred (\tau_i) \implies st_i \geq ft_j
\end{align}
%\begin{align}
%&\forall \tau_i \And \forall j\in Pred (\tau_i) \implies st_i \geq ft_j
%\end{align}

\textit{Mapping Constraint:} A task ($\tau_i$) can only be executed on a single core in each time slot. If $X_{ij}$ denotes the mapping of task $\tau_i$ on core $j$, then:
\begin{align}
 \forall \tau_i, \sum_{j \in Cores}{X_{ij}} = 1  
\end{align}

\begin{table*}[ht]
	\centering
	\caption{All possible scenarios of executing the task graph presented in \figureRef{fig:a_taskGraph} on a single core chip}
	\begin{threeparttable}
		\begin{tabular}{ccccccccccccccc}
			\toprule
			\multirow{1}{1cm}{\centering \textit} &
			\multirow{1}{0.6cm}{\centering $S_1$ }&
			\multirow{1}{0.6cm}{\centering $S_2$ }&
			\multirow{1}{0.6cm}{\centering $S_3$ }&
			\multirow{1}{0.6cm}{\centering $S_4$ }&
			\multirow{1}{0.6cm}{\centering $S_5$ }&
			\multirow{1}{0.6cm}{\centering $S_6$ }&
			\multirow{1}{0.6cm}{\centering $S_7$ }&
			\multirow{1}{0.6cm}{\centering $S_8$ }&
			\multirow{1}{0.6cm}{\centering $S_9$ }&
			\multirow{1}{0.6cm}{\centering $S_{10}$ }&
			\multirow{1}{0.6cm}{\centering $S_{11}$ }&
			\multirow{1}{0.6cm}{\centering $S_{12}$ }&
			\multirow{1}{0.6cm}{\centering $S_{13}$ }&
			\multirow{1}{0.6cm}{\centering $S_{14}$ }\\
			\midrule
			\multicolumn{1}{c}{Overrun}	&\multicolumn{1}{c}{-}	&\multicolumn{1}{c}{-}	&\multicolumn{1}{c}{-}	&\multicolumn{1}{c}{-}	&\multicolumn{1}{c}{$T_1$}	&\multicolumn{1}{c}{$T_2$} &\multicolumn{1}{c}{$T_1$\tnote{*}~\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}	&\multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}} 	&\multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}	&\multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}  &\multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}	&\multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}	&\multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}} 	&\multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}  \\
			\multicolumn{1}{c}{Fault}					& \multicolumn{1}{c}{-}	& \multicolumn{1}{c}{$T_1$}	&	\multicolumn{1}{c}{$T_2$}	& \multicolumn{1}{c}{$T_3$}	& \multicolumn{1}{c}{-}		& \multicolumn{1}{c}{-} 	& \multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}	& \multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}} 	& \multicolumn{1}{c}{$T_3$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}	& \multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}  & \multicolumn{1}{c}{$T_3$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {2}}}}	& \multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}}	& \multicolumn{1}{c}{$T_1$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}} 	& \multicolumn{1}{c}{$T_2$\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {1}}}} 	\\
			\multicolumn{1}{c}{Finish time}	&\multicolumn{1}{c}{9}	& \multicolumn{1}{c}{14}	&	\multicolumn{1}{c}{13}		& \multicolumn{1}{c}{12}	&\multicolumn{1}{c}{13}	& \multicolumn{1}{c}{11} & \multicolumn{1}{c}{\textbf{20}\tnote{***}}	 													& \multicolumn{1}{c}{\textbf{19}\tnote{***}} 														& \multicolumn{1}{c}{16}														& \multicolumn{1}{c}{17}  							& \multicolumn{1}{c}{12}	& \multicolumn{1}{c}{18}	& \multicolumn{1}{c}{16} 	& \multicolumn{1}{c}{15}  \\
			\multicolumn{1}{c}{Exe time (drop $T_3$)}	& \multicolumn{1}{c}{7}	 	& \multicolumn{1}{c}{12}	&	\multicolumn{1}{c}{11}		& \multicolumn{1}{c}{10\tnote{**}}	& \multicolumn{1}{c}{11}	& \multicolumn{1}{c}{9} & \multicolumn{1}{c}{18}	 & \multicolumn{1}{c}{17} 			& \multicolumn{1}{c}{14\tnote{**}}		& \multicolumn{1}{c}{15}  							& \multicolumn{1}{c}{10\tnote{**}}	& \multicolumn{1}{c}{16}	& \multicolumn{1}{c}{14} 	& \multicolumn{1}{c}{13}  \\
			\bottomrule
		\end{tabular}%
		\begin{tablenotes}
			\item[*] {\footnotesize The circles shows the order of the occurrence of fault and task overrun.}
			\item[**] {\footnotesize In these cases, the system executes $T_3$ and detects a fault occurs, but does not re-execute the task (drops the task).}
			\item[***] {\footnotesize In these cases, the system must drop task $T_3$ to execute all HC tasks before their deadlines.}
		\end{tablenotes}
	\end{threeparttable}
	\label{tab:Motivational}%
\end{table*}%



\textit{Power Constraint:} The chip's overall power consumption must not violate the chip's TDP~($TDP_{chip}$) in any time slot.%of the chip
\begin{align}
 & \forall t \in timeslots: \sum_{j \in Cores}{Pow_{jt}} \leq TDP_{chip},  
\end{align}
where $Pow_{jt}$ represents the power consumption of core $j$ in time slot $t$.

%Since some LC tasks may be dropped in the HI mode to solve the problem and meeting the timing constraints, the LC tasks' QoS should be improved when the system switches to the HI mode.
When the system switches to the HI mode, the system drops some LC tasks to meet the timing constraints, which degrades the QoS of the system:
\begin{align}
 &Cr_L= HI: \quad QoS = n_L^{succ}/n_L 
\end{align}


The problem is how to map and schedule dependent MC tasks of application A on the system's cores to satisfy the aforementioned constraints (timing and peak power) and QoS of the system.
In this paper, we propose a heuristic method to solve this NP-hard problem \cite{munawar14}.

%As a result, the problem is how to map and schedule dependent MC tasks of application \textit{A} on cores that the above constraints are satisfied, the QoS is improved and also, the maximum temperature of the processor is managed by the proper task mapping to prevent hot spots in the chip. Since the problem is classified as an NP-hard problem~\cite{munawar14}, a heuristic method is proposed, which is presented in the next section.
%In the following, we propose our method in detail.


==> Sections/PPMethodFinal.tex <==

\section{PROPOSED METHOD}
\label{sec:proposalMethod}

In this section, at first, a motivational example is presented in Section~\ref{subsec:motivationalExample} for a better understanding of the problem and the proposed solution. 
Then, the proposed method is explained in detail in Section~\ref{subsec:Method} and~\ref{subsec:treeConstructionStrategies}.



\subsection{Motivational Example}
\label{subsec:motivationalExample}


\figureRef{fig:a_taskGraph} shows an application with three tasks, where tasks ${T}_{1}$ and ${T}_{2}$ have HC, and task ${T}_{3}$ has LC.
Deadline, low WCET, and high WCET of each task are presented in the figure, and the system takes 1ms to discard the output of a faulty task ($\mu=1$). Hence, the period of all tasks are the same and is equal to \textit{18}ms. 
For the sake of simplicity, we considered that the application runs on a single-core processor, and up to one fault may occur during the execution of the application ($k=1$). 
So, the system cannot execute multiple tasks simultaneously on different cores to violate TDP (we will discuss TDP challenge later). 
The scheduling algorithm in the LO mode, executes tasks $T_1$, $T_2$, and $T_3$, respectively. 
The schedulability test~\cite{baruah16} shows that in the LO mode, all three tasks can be executed even in the case of fault occurrence. In other words, the total CPU utilization for application $A$ is less than one $(U_{A} \leq 1)$. 
If we consider the HI mode, if a LC task $T_3$ is executed in addition to the two HC tasks in the case of fault occurrence, the system becomes overloaded~($U_A^{HI}$>1) and the three tasks cannot be scheduled. However, if we drop some LC tasks in the HI mode ($T_3$ in this example) to guarantee the correct execution of HC tasks, then the computation demand requested by tasks is less than one and can be scheduled before their deadline. As a result, the utilization of this example for both LO and HI modes with the probability of one fault occurrence is computed as follows, in which, just LC tasks are considered to be executed in the HI mode.
\begin{align}
\label{eq:3}
\begin{split}
U_A &= MAX(U_A^{LO}, U_A^{HI}) \leq 1 \\
U_A^{LO} &= (\sum_{i \in \lbrace 1,2,3\rbrace} \frac{C_i^{LO}}{P_A})
+\frac{k(\max_{i \in \lbrace 1,2,3\rbrace}(C_i^{LO}) +\mu)}{P_A}\\
&=\frac{4}{18}+\frac{3}{18}+\frac{2}{18} +(\frac{4+1}{18})=\frac{14}{18}<1 \\
U_A^{HI} &= (\sum_{i \in \lbrace 1,2\rbrace} \frac{C_i^{HI}}{P_A})+\frac{k(\max_{i \in \lbrace 1,2\rbrace}(C_i^{HI}) +\mu)}{P_A}\\
&=\frac{6}{18}+\frac{5}{18}+(\frac{6+1}{18})=\frac{18}{18} \leq 1
\end{split}
\end{align}




However, for this example, fourteen different scenarios could happen during the execution of the application because the time of the fault and task overruns are unknown.
\tableRef{tab:Motivational} shows all these scenarios, and the execution time of the system whether it drops LC task or not.
In ten scenarios ($S_5$ to $S_{14}$), an HC task overruns, and it shows the system is in the HI mode.
However, as shown in \tableRef{tab:Motivational}, only in two scenarios, the system fails to execute all tasks (HC and LC tasks) before the deadline ($S_7$ and $S_8$). The reason is that, the system has switched to the HI mode in these scenarios and also a fault has occurred. it causes the system to be overloaded and the computation demand for executing all tasks becomes more than one~($U_A>1$). Therefore, the LC task $T_3$ would be dropped. Although there are some scenarios such as $S_{12}$ to $S_{14}$, that the system is in the HI mode, we schedule the LC task in this mode to improve the QoS. As shown in \tableRef{tab:Motivational}, the start time of $T_3$ in $S_{12}$ ($S_{14}$) is 16 (13), and since the WCET of the LC task is 2, then it can be executed before the application deadline ($d_A=18$).
This example clearly shows that all situations should be considered in an MC system. Therefore, the system is analyzed in detail at design-time, and then, the proper schedule is exploited in the online phase to minimize the drop ratio of LC tasks and enhance the QoS.% of the system.


\begin{figure}[!t]
	\centering
	\includegraphics[width=1\columnwidth]{imgs/TGFig2.pdf}
	\caption{Task graph of an application with three tasks used in the example}
	\label{fig:a_taskGraph}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.73\columnwidth]{imgs/TreeAllSennew.pdf}
	\caption{The tree constructed by our method for the task graph of \figureRef{fig:a_taskGraph}}
	%\caption{The tree constructed by the proposed method for the task graph presented in \figureRef{fig:a_taskGraph}.}
	\label{fig:b_scheduleTree}
\end{figure}

\figureRef{fig:b_scheduleTree} shows the tree for the application task graph presented in the motivational example, which is constructed in the offline phase of our proposed approach.
At run-time, the system starts each period with $S_1$ (the scheduling in the root of the tree), which corresponds to the scenario where no fault occurs and no HC tasks overruns. 
If an HC task overruns (for instance task $T_1$), The system searches through the children of the current node ($S_1$), finds the appropriate task mapping and scheduling, and continues the execution based on the new schedule ($S_6$ in this case). 
After that, if error detection unit detects a fault at the end of a task execution (for instance task $T_2$), the system searches through the children of the current node ($S_6$), finds the appropriate scenario, and continues the execution based on the new task mapping and scheduling ($S_{14}$ in this case).




It is important to mention that each schedule has a different start time, system mode, the expected number of faults, and task set.
Furthermore, scheduling of child nodes must be compatible with the scheduling of their parent; so, the system can change the schedule of tasks without any conflicts. 
For instance, assume that in $S_1$, the task execution order is $T_1$, $T_2$, and $T_3$. 
When the system employed $S_4$, it implies that $T_1$ and $T_2$ are completed successfully, the system is in the LO mode, and a fault is detected at the end of the first execution of $T_3$. 
So, the $S_4$ should schedule tasks based on this information.
%In the following subsection, we explain how the scheduling tree is generated.

%\begin{figure}
%\begin{minipage}[b]{1\linewidth}
%\centering
%\renewcommand{\thesubfigure}{C-1}% New fixed/manual numbering
%\subfloat[Schedule S1]{\label{fig:c_1}\includegraphics[1\linewidth]{imgs/C1.pdf}}
%\renewcommand{\thesubfigure}{C-2}% New fixed/manual numbering
%\subfloat[Schedule S6]{\label{fig:c_2}\includegraphics[1\linewidth]{imgs/C2.pdf}}
%\renewcommand{\thesubfigure}{C-3}% New fixed/manual numbering
%\subfloat[Schedule S12]{\label{fig:c_3}\includegraphics[1\linewidth]{imgs/C3.pdf}}
%\renewcommand{\thesubfigure}{C-4}% New fixed/manual numbering
%\subfloat[Schedule S9]{\label{fig:c_4}\includegraphics[1\linewidth]{imgs/C4.pdf}}
%\end{minipage}
%\caption{Scheduling tree and their different scenarios}
%\label{fig:main}
%\end{figure}


\subsection{Design Methodology}
\label{subsec:Method}

The fault-tolerance and peak power-aware task mapping and scheduling method consists of two phases, design-time, and run-time. In this paper, we focus on system design at design-time. For the sake of completeness, we provide a brief overview of how to use the schedule tree in the run-time phase, which is generated at design-time. Fig.~\ref{fig:method} shows an overview of the design methodology. In the design-time phase, there are three functions which are used to generate the schedule tree, \textit{MakeTreeRec}, \textit{Schedule}, and \textit{MapSch}. Section~\ref{subsec:treeConstructionStrategies} provides details of generating the tree, these functions, and how we manage the peak power consumption. All scenarios are stored in memory to be used in the run-time phase. At run-time, an application follows the presented task mapping and scheduling in the root of the tree. In the case of fault occurrence or mode switching, the appropriate task mapping and scheduling for the remaining un-executed tasks are fetched from memory. After fetching, mapped tasks based on the previous scenario are re-mapped based on the new scenario, and the system continues its operation. In the following subsection, we explain the design-time phase of our proposed method. 



%\subsection{Scheduling Tree Generation and Fault-Tolerant Scheduling and Mapping}
\subsection{Tree Generation and Fault-Tolerant Scheduling \& Mapping}
\label{subsec:treeConstructionStrategies}


As we discussed, multiple scenarios might happen during the execution of an instance of the application, where, in most of these scenarios, the system can execute all or most of LC tasks without violating HC tasks' deadline.
To this end, the proposed approach of this paper considers a different mapping and scheduling for each scenario to handle HC tasks deadlines, faults, and peak power violations while minimizing the number of dropped LC tasks in the HI mode.
In the run-time phase, in general, the system is unaware of tasks that might overrun or a fault occurs; so, the system cannot select the proper schedule in advance.
Therefore, this paper employs a tree data structure in the offline phase to organize the mapping and scheduling of tasks for all scenarios, corresponding to~each HC task overrunning, and/or up to $k$ faults occurrence during each period. Now, we explain how the scheduling tree is generated.

\begin{figure}
	\centering
	\includegraphics[width=1\columnwidth]{imgs/drawnew.pdf}
	\caption{Design methodology}
	\label{fig:method}
\end{figure}


\subsubsection{\textbf{Making Scheduling Tree}}

The main function of creating the tree ($\Phi$) is outlined in Algorithm~\ref{alg:schedulingTree}.
At first, we define a priority queue called \textit{TaskPQ} (line 3), which considers tasks' release time as the priority.
The release time of a task is the time when all its predecessor tasks have finished their execution (presented in Section \Ref{subsec:mixedCriticalityTaskModel}).
Then, the algorithm enqueues all tasks without any predecessor to the \textit{TaskPQ} with key equal to 0; because they are released at the beginning of the period (line 4).
Each node of the tree represents a particular scenario, and it has two attributes called \textit{sch} and \textit{childs}.
For instance, in the root scenario, the system is in the LO mode, and no fault occurs in the entire period.
\textit{sch} is the proper mapping and scheduling of tasks for that scenario, and \textit{childs} is a list of children nodes of the current node.

\begin{algorithm}[!t]
\footnotesize
		\caption{Creating the Tree}
		\label{alg:schedulingTree}
		\begin{threeparttable}
				\begin{algorithmic}[1]
					\renewcommand{\algorithmicrequire}{\textbf{Input:}}
					\renewcommand{\algorithmicensure}{\textbf{Output:}}
					
					\Require Task Graph ($G_{T}$), List of Cores ($c$), Number of Faults ($k$).
					\Ensure Scheduling Tree ($\Phi$).

					\Procedure{MakeTreeMain}{}
					\State $\Phi \gets$ Empty Tree
					\State \textit{TaskPQ} $\gets$ Empty Priority Queue
					\State Add all tasks without predecessor node to \textit{TaskPQ} with key $0$
					\State $\Phi[root].sch \gets MapSch (G_{T}, c, 0, \varnothing, TaskPQ)$ 
					\If {$\Phi[root].sch$=\textit{un-scheduled}}
					\State \Return {$\varnothing$}
					\EndIf
					\State $\Phi[root].childs \gets MakeTreeRec (G_{T}, c, $\algbrakline{4.5}$\Phi[root].sch, 0, k, LO)$
					\If {$\Phi[root].childs$=\textit{un-scheduled}}
					\State \Return {\textit{un-scheduled}}
					\EndIf
					\State \Return {$\Phi$}
					\EndProcedure
					
					\Function{MakeTreeRec}{Task Graph ($G_{T}$), List of Cores ($c$), Parent Schedule($Sch$), Time ($T$), Number of Faults ($k$), Mode of the System ($Mode$)}

					\State \textit{SchList} $\gets$ Empty list of nodes
					
					\If {\textit{Mode} = \textit{LO}} // \textit{HChild} nodes
					\State \textit{Tasks} $\gets$ List of unfinished HC tasks in time \textit{T}.
					\State $G_{H} \gets$ $G_{T}$ With High WCET.
										
					\ForEach {$\tau$ \textbf{in} \textit{Tasks}} 
					\State $T_{tmp} \gets$ Finish time of $\tau$ in \textit{sch} + $T_{sw}$.
					\State S $\gets$ New node
					\State S.sch = {\textit{Schedules}} ($G_{H}$, c, $T_{tmp}$, \textit{sch}, \textit{TaskPQ})
					\If {S.sch = un-scheduled}
					\State \textbf{return} $\varnothing$.
					\EndIf		
					\State $S.childs \gets MKTreeRec (G_{H}, c, S, T_{tmp}, k, HI)$
					\If {$S.childs = \varnothing$}
					\State \textbf{return} $\varnothing$.
					\EndIf	
					\State Add $S$ to $SchList$			 				
					
					\EndFor	
					\EndIf
					
					\If {\textit{k} $>$ 0}
					\State \textit{Tasks} $\gets$ List of Unfinished Tasks in \textit{T}.
					
					\ForEach {$\tau$ in \textit{Tasks}} 
					\State $T_{tmp} \gets$ Finish Time of $\tau_{i}$ in \textit{sch}.
					\State S.sch = {\textit{Schedules}}({$G_{T}$,~\textit{sch},~\textit{Time}})
					\If {S.sch = un-scheduled}
					\State \textbf{return} un-scheduled.
					\EndIf						
					
					\State $S.childs \gets MKTreeRec (G_{T},c,S, T_{tmp},k-1, Mode)$
					\If {$S.childs = \varnothing$}
					\State \textbf{return} $\varnothing$.
					\EndIf
					\State Add $S$ to $SchList$			 						
					
					\EndFor	
					\EndIf
					
					\State \Return{$SchList$}
					\EndFunction					
					
					
			 	\end{algorithmic}
		\end{threeparttable}
\end{algorithm}




The algorithm calls \textit{MapSch} function (Algorithm~\ref{alg:mapsche}, which is discussed later in Section~\ref{subsubsec:MapandSch}) to schedule task for the root node (line~5).
The algorithm returns \textit{un-scheduled}, if \textit{MapSch} function cannot find any feasible schedule with no task dropping and violating the TDP constraint (lines 6-8).
Otherwise, the algorithm in line 9 continues to create the rest of the tree recursively by calling \textit{MakeTreeRec} function (which is presented in lines 15-50 of this algorithm).
If task scheduling is feasible in all possible scenarios, \textit{MakeTreeRec} function returns a list of child nodes, and the algorithm returns the tree ($\Phi$); otherwise, the algorithm returns \textit{un-scheduled} which means it could not find a feasible solution (lines 10-13). 


The \textit{MakeTreeRec} function in Algorithm~\ref{alg:schedulingTree} recursively creates the tree.
Each node in the tree might have two types of child nodes.
The first type of child node (\textit{HChild}) has a scenario similar to their parents, except that one of the HC tasks overruns. 
%In MC systems, when an HC task overruns and the system switches to the HI mode, the scheduler considers the high WCET of all remaining HC tasks until the end of the period~\cite{baruah16,Medina18}. 
Therefore, if the system is in the LO mode, any unfinished HC task might overrun and change the system's mode.
To this end, first, \textit{MakeTreeRec} function collects all unfinished HC tasks and creates an HC task graph ($G_H$) by changing the WCET of all tasks to high WCET (lines 18-19). 
Then, for each unfinished HC task, the function considers the scenario that the task overruns and schedules the task by calling \textit{Schedules} function, presented in Algorithm~\ref{alg:schedulingTree2}.
If the \textit{Schedules} function finds feasible scheduling, the algorithm recursively creates a tree for this node, where the system is in the HI mode, and up $k$ faults may occur on the remaining tasks by calling \textit{MakeTreeRec} function (lines 20-32). 
It is important to mention that switching to the HI mode has non-zero timing overhead ($T_{sw}$) in realistic systems~\cite{Chisholm17}, but it is insignificant in comparison with tasks' WCETs (line 21). 
The second type of child node (\textit{FChild}) has a scenario similar to their parents, except one fault occurs during the execution of one of the remaining tasks.
As we mentioned in \sectionRef{subsec:faultTolerantModel}, the system can tolerate up to $k$ faults in a period.
If less than \textit{k} faults occur in a node scenario, a faulty execution of all remaining tasks needs to be considered. 
Therefore, a child node is generated for the faulty execution of each remaining task, and also for each child node, the algorithm recursively constructs a tree by calling \textit{MKTreeRec} with \textit{k-1} faults (line 34-48).
Finally, if the algorithm finds a feasible solution for all scenarios, it returns the list of child nodes ($SchList$).


\begin{algorithm}[!t]
	\footnotesize
	%	\begin{changedEnv}
	\caption{Schedule Procedure}
	\label{alg:schedulingTree2}
	\begin{threeparttable}
		\begin{algorithmic}[1]
			\renewcommand{\algorithmicrequire}{\textbf{Input:}}
			\renewcommand{\algorithmicensure}{\textbf{Output:}}				

					\Require Task Graph ($G_{T}$), List of Cores ($Cores$), Time ($T$), Parent Schedule ($Sch_{par}$), Ready Task Priority Queue ($TaskPQ$).
					\Ensure Schedule ($Sch$)

					\Procedure{Schedules}{}			
					\State $T_{r} \gets$ List of Tasks from $G$ that all predecessors \algbrakline{1.15} has started executing before time \textit{T}.
					
					\State Add $T_{r}$ Tasks to a Priority Queue (\textit{TaskPQ}).
					
					\State $Sch \gets Sch_{par}[0-T]$
					\State $Sch \gets MapSch (G_1, Cores, T, Sch, TaskPQ)$
					\If {$Sch$ = un-scheduled}
					\State Find a LC Task with Largest execution time which has not started \algbrakline{0.8} in \textit{T} and remove it from $G$ then \textbf{goto} line 2.
					\If {Cannot find any LC task} 
					\State \textbf{return} un-scheduled.
					\EndIf
					\EndIf					
					\State \textbf{return} $Sch$
					\EndProcedure
			
		\end{algorithmic}
	\end{threeparttable}
\end{algorithm}




%It is noteworthy to mention that t
The \textit{Schedule} function, schedules tasks for each situation by calling \textit{MapSch} function (Algorithm~\ref{alg:mapsche}).
If \textit{MapSch} function fails to find a feasible solution to meet the deadlines of all tasks with respect to TDP constraint, \textit{Schedules} function drops the largest LC task (in terms of WCET) and calls \textit{MapSch} function again.
The \textit{Schedules} function repeats this procedure to find a feasible schedule.
If \textit{MapSch} function fails to find a feasible solution, and there is no more LC task to drop, \textit{Schedules} function returns \textit{un-scheduled} (lines 2-12 Algorithm~\ref{alg:schedulingTree2}).
We will discuss the \textit{MapSch} function in the next subsection.
As we mentioned in this section, occurring faults and a criticality mode change generate different scheduling scenarios that correspond to a set of alternative schedules.
These scenarios are stored in the memory of the system as a tree in the offline phase. 
At run-time, the system starts with the scheduling in the root node, which is for the scenario that no fault or overrun happens.
After that, if a fault occurs or an HC task overruns, the system finds the appropriate scenario in the child nodes of the current node and changes the scheduling of the system to improve the number of executed LC tasks.


%\algorithmRef{alg:schTreeOrg} shows the pseudo code of how the tree is generated. The schedules should be created for all scenarios that tasks are overrun or faults occur. At first, the root of the tree is created which is the state that no fault occurs in the LO mode. At the beginning, we set the scheduling tree, as an empty list (line 2). %schedule $S_{1}$ is created (it will be the root of the tree), which is the state that no fault occurs in the low-criticality mode (line 2).
%We generate the possible schedules in two parts. It should be mentioned that we use recursively approach to construct the scheduling tree. At first, The system starts in the LO mode. We define a list (\textit{HCT}) which contains an unfinished high-criticality tasks in the task graph (line 4). Each high-criticality task may overrun. If a task is overrun, WCET of this task and the remaining high-criticality tasks will be equal to ${C}_{i}^{HI}$ (line 6). So, we generate all possible scenarios that each high-criticality task overruns and add them to the list (line 5-14). \fixme{Also, all possible scenarios generated by these considered scenarios are added after the investigated scenarios (line 12, 13). Actually, they generate recursively.}
%Each investigated scenario is added to the list and  %(line 15, 27). 
%As we discussed, possible scenarios are generated due to the fault occurrence (line 16-27). % and mode switching (line 3-15).
%All tasks is followed in the graph and all the possible schedules are generated by considering utmost \textit{k} faults. This part generated schedules recursively, too. Actually, this flow is done until all possible scenarios are investigated. If one of these scenarios is unschedulable, the tree cannot be generated for the task graph (line 9-11, 21-23). 

%\algorithmRef{alg:mapsche} is used to map and schedule tasks for each scenario in calling \textit{schedules} function (line 34). It should be mentioned that if a fault occurs during the execution of a task, the task will be re-executed to recover from a fault. This state is considered in calling \algorithmRef{alg:mapsche} in each scenario. Also, when a high-criticality task is overrun or a fault occurs, it may affect on peak power consumption or execution time of the other tasks. The execution of low-criticality tasks can be stopped in the HI mode due to the deadline meeting of high-criticality tasks and peak power management in this situation. One target of proposed algorithm %(which is considered in \algorithmRef{alg:mapsche}) 
%is that more low-criticality tasks are executed in the HI mode due to the QoS maximization while deadlines of all tasks are met. So, if low-criticality tasks should be dropped, we find one that has largest WCET and drop it (line 35-40). If there is no low-criticality task to drop, this task graph is unschedulable in this situation (line 37-39).
%We should consider all possible scenarios to develop the scheduling tree.
	
%As we mentioned in this section, occurring faults and a criticality mode change generate different scheduling scenarios that correspond to a set of alternative schedules. These scenarios are in a database that is a tree structure and a proper schedule is selected easily according to the situations, in runtime.

%The purpose of this proposed algorithm is to generate a scheduling tree for task graphs like \figureRef{fig:b_scheduleTree}. This tree includes different schedules that are generated considering that up to \textit{k} transient faults may occur during the execution of the application and the system situation in different criticality modes. The root of the tree is a schedule of the condition where no fault occurs in the LO mode.

%The pseudo code of our proposed algorithm for generating the scheduling tree ($\Phi$) is outlined in \algorithmRef{alg:schedulingTree}. At first, we define a queue (called \textit{TaskPQ}), which contains ready tasks that are released (line 3). At the begining, the root of the task graph is in this queue (line 4). We do two steps to develop this tree. In the first step, we check the feasibility of task scheduling assuming no fault occurrence (line 5-8). In this step, it is checked that all tasks in the task graph finish correctly before their deadlines. If there is a task causing the TDP violation or missing deadline of other tasks, this application is not schedulable. It should be mentioned that, this scheduling algorithm determines the start time and the order of tasks that the TDP constraint of the chip is not violated. Also, we determine that each task is executed on which core to prevent the emergence of hotspots. It is also checked that the deadlines of the tasks do not miss and the TDP constraint of the system is not violated. The details are proposed in \algorithmRef{alg:mapsche}. 
%In the second step, the feasibility of high-criticality task scheduling in the high-criticality mode is checked without considering fault occurrence probabilities (line 3). If there is at least one high-criticality task missing its deadline in the high-criticality mode, the application is not schedulable (line 4). In this step, low-criticality tasks can be dropped to provide the opportunity of meeting the deadline of the high-criticality tasks. 
%The last step is to generate the scheduling tree by considering \textit{k} transient fault occurrence and a criticality mode change (line 9-12). The details of this algorithm are presented in \algorithmRef{alg:schTreeOrg}.

\begin{algorithm}[!t]
\footnotesize
	%\begin{changedEnv}
		\caption{Mapping and Scheduling Pseudo Code}
		\label{alg:mapsche}
		\begin{threeparttable}
			{ \small
				
				\begin{algorithmic}[1]
					\renewcommand{\algorithmicrequire}{\textbf{Input:}}
					\renewcommand{\algorithmicensure}{\textbf{Output:}}
					
					\Require Task Graph ($G_{T}$), List of Cores ($Cores$), Time ($T$), Scedule up to the Time ($Sch$), Ready Task Priority Queue ($TaskPQ$).
					
					\Ensure Complete Schedule ($Sch$)
					
					\Procedure{MapSch}{}
					    
					    \For {\textit{TS} = $T$ \textbf{to} \textit{PERIOD}}
					        \State $ReadyTasks \gets \varnothing$
					        
					        \State Extract minimum element from \textit{TaskPQ} and add it
					        to  \par
					        \hskip\algorithmicindent
					        \textit{ReadyTasks} while key of each element is equal to \par
					        \hskip\algorithmicindent \textit{TS} and \textit{TaskPQ} is not empty;
					        
					        \If{\textit{TaskPQ}.empty() = \textbf{true} \textbf{and} \textit{ReadyTasks} $= \varnothing$}
					        \State \Return $Sch$ \textit{//} Scheduling is done;
					        \EndIf

					        
					        \If{\textit{ReadyTasks} $= \varnothing$}
					            \State \textbf{continue} \textit{//} No new task is ready in this \textit{TimeSlot}
					       \EndIf				       
					            

					      \State \textit{SortedTasks} $\gets$ Sort (\textit{ReadyTasks, Desc}); %// Energy Con.%Eq.~\ref{eq:CostF_Task}
                          \State \textit{SortedCores} $\gets$ Sort (\textit{Cores, Asc});% // Eq.~\ref{eq:CostF_Core}
                                
                                
                                \For {\textit{task} \textbf{in} \textit{SortedTasks}}
                                    \For {\textit{core} \textbf{in} \textit{SortedCores}}
                               \State $\textit{Time}_\textit{tmp} \gets \textit{task}_\textit{wcet}$
                               
                               \State $count \gets 0$

                               \State $Sch_{tmp} \gets Sch$
                               
                               \State $SysPow_{tmp} \gets SysPow$

                               
                                \While {$Time_{tmp}$ > $0$}
                                 
                                \If{$Sch_{tmp}(TS$+$count, core)$ is empty \& \algbrakline{1.2} $SysPow_{tmp}(TS$+$count)$ + $task_{pow}$ <= $TDP$}
                                
                                   \State $Sch_{tmp}(TS+count, core)$ = $task$
                                   
                                   \State $SysPow_{tmp}(TS+count)$ += $task_{pow}$
                                   
                                   \State $Time_{tmp}$ -= $1$ 
                                    
                        %        \EndIf
                                \EndIf
                                \State $count$ += $1$;
                                \EndWhile
                                 
 
                              \If{$TS$+$count \leq task_{deadline}$} 
                                \State $Sch \gets Sch_{tmp}$
                               
                               \State $SysPow \gets SysPow_{tmp}$

                              
                            %  \State $\textit{core}_\textit{FTime} \gets TS$+$count$
                                
                                \State \textit{SortedCores} $\gets$ Sort (\textit{Cores, Asc}); %// Eq.~\ref{eq:CostF_Core}
                         \State $task_{sch} \gets $ \textbf{true}
                                \State \textbf{break}
                             \EndIf 
                                
                                    \EndFor
                            
                                  
                                    
                             \If{$task_{sch}$ == \textbf{false}}
  
                                           \State \Return {un-scheduled}

                                        \EndIf                  

                                        
                                \EndFor                                


				    \EndFor                        
					\EndProcedure
				\end{algorithmic}
			}
		\end{threeparttable}
	%\end{changedEnv}
\end{algorithm}



\subsubsection{\textbf{Mapping and Scheduling}}
\label{subsubsec:MapandSch}
In this section, we explain the proposed mapping and scheduling algorithm, which manages the peak power and hotspot distribution.
It should be mentioned that low power techniques, e.g., DVFS, cannot be easily used in the HI mode, especially when the system is in the overload situation due to the timing overhead. Therefore, we manage the peak power by finding the proper mapping and scheduling of tasks on free time slots of cores. This task mapping and scheduling are feasible if the system's power consumption never exceeds the TDP constraint, and all tasks finish their execution (even in the worst case) before their deadline.
So, \textit{MapSch} algorithm decides the time and core where each task should be executed.


%%Pseudo-Code

Algorithm~\ref{alg:mapsche} outlines the pseudo-code of the \textit{MapSch} algorithm.
\behnaz{Tasks are mapped and scheduled up to time \textit{T} based on the current node schedule. In the case of fault occurrence or mode switches at time \textit{T}, this algorithm maps and schedules the rest of the tasks based on the new node schedule from time \textit{T} to the end of the application period (\textit{PERIOD}).}
%Tasks are mapped and scheduled up to time \textit{T}, and this algorithm will map and schedule the rest of the tasks from time \textit{T} to the end of the application period (\textit{PERIOD}). 
The time is divided into a set of equal time slots (\textit{TS}), and the scheduler will put tasks into cores only at the beginning of each time slot.
In each time slot, at first, the algorithm sets an empty array for ready tasks, and then it extracts all elements of \textit{TaskPQ}, where their key is equal to the current time slot. This means that all predecessor tasks of these ready tasks have finished their execution. If \textit{TaskPQ} and \textit{ReadyTasks} array are both empty, the algorithm returns the final scheduling (\textit{Sch}) because it successfully schedules all tasks. 
If there is no ready task to be scheduled in the current time slot (the \textit{ReadyTask} array is empty, but the \textit{TaskPQ} is not empty), the algorithm moves to the next time slot (lines~2-10).




The algorithm sorts the ready tasks in descending order of their energy consumption (line 11). 
The energy consumption of each task $\tau_i$ ($Eng_i$) is calculated as follow:
\begin{align}
Eng_i=Pow_i\times~WCET_i  
\end{align}
where $Pow_i$, and $WCET_i$ are the maximum power consumption, and the worst case execution time of task $\tau_i$. 
The maximum power of each task can be obtained by running benchmarks on a real platform. As mentioned in Section~\ref{PowModel}, the processor power consists of three components; when a task is run on a processor, the dynamic power is increased significantly compared to static and independent powers. Hence, in this paper, we don't model the power; we measure the processor power when task are run on the real platform. More information about computing these values is given in Section~\ref{subsec:experimentalSetup}. \behnaz{The system's power consumption must never exceed the TDP constraint to overcome to overheating problem~\cite{Ansari2018,munawar14}. To this end, we consider a constant power~consumption for each task at design-time, which is equal to its maximum power consumption, to guarantee the meeting of TDP constraint in the worst-case scenario.}
In addition, energy increment leads to an increase in chip temperature~\cite{huang14,Ranjbar2020}. Thus, we map a task with more energy consumption to a core with less temperature. Then, the algorithm sorts the cores in the ascending order of their accumulated energy (line~12). A core has a higher priority for task assignment if it has~less accumulated energy (i.e., tends to have a less temperature degree).

\begin{figure*}

\centering

%\subfloat[Task graph example]{\includegraphics[width=0.25\textwidth]{imgs/TGExample_a.pdf}\label{fig:fig5a}}
\subfloat[An example of MC application]{\includegraphics[width=0.33\linewidth]{imgs/Fig5a-PPM.pdf}\label{fig: example application}}
\hspace{0.5cm}
\subfloat[Task scheduling without our policy]{\includegraphics[width=0.29\linewidth]{imgs/fig4newb.pdf}\label{fig:fig5b}}
\hspace{0.5cm}
\subfloat[Task scheduling with our policy]{\includegraphics[width=0.29\linewidth]{imgs/fig4newc.pdf}\label{fig:fig5c}}

\caption{Two different task scheduling scenarios}% for Task Graph in \figureRef{fig: example application}}
\label{fig:scheduling5}
%\vspace{-10pt}
\end{figure*}



After sorting tasks and cores, the algorithm assigns tasks to the cores one by one (lines 13-38).
So, for each task, the algorithm selects a core from the sorted list and schedules~the task on the core's free slots (lines 19-26). 
The system's~instantaneous power consumption must be less than the TDP constraint; so, we consider an array called $SysPow$, which holds the maximum power consumption of the system in each time slot.
The algorithm checks the $SysPow$ and TDP constraint before scheduling a task on a core (line 20). If the task is completed before its deadline, the algorithm updates the schedule ($Sch$), power array ($SysPow$), and scheduling~status of the task ($task_{sch}$). It also sorts the cores again since the energy of one core has changed, and starts to schedule the next task (lines 27-33). If the task does not meet its deadline on the core, the algorithm picks the next core and schedule it on that core. However, if the deadline of one task is violated in all cores, the algorithm fails to schedule tasks of the application in this scenario and returns "un-schedulable" (lines 36-37). % all tasks of the application in this scenario and returns "un-schedulable" (lines 36-37). 

%If the task is completed before its deadline, the algorithm updates scheduling($Sch$), power array ($SysPow$), the finish time of the core($FinTime_c$), and scheduling status of the task ($task_{sch}$). It also sorts the cores again since the finish time of one core has changed, and start to schedule the next task (lines 27-34). If the task does not meet its deadline on the core, the algorithm picks the next core and schedule the task on that core. However, if the deadline of one task is violated in all cores, the algorithm fails to schedule all tasks of the application in this scenario and returns "un-schedulable" (lines 36-37). 


The example in Fig.~\ref{fig:scheduling5} shows an MC application and how our method maps and schedules the tasks on three cores. 
Assume the TDP constraint is 1.6 Watt. Fig.~\ref{fig:fig5b} shows that the scheduling without our policy violates the TDP constraint, while the maximum power consumption of the task scheduling by considering our policy is below the TDP constraint (Fig.~\ref{fig:fig5c}). 
When the system completes task $T_1$, three tasks ($T_2$, $T_3$ and $T_4$) become ready to be executed.  %So, considering $\beta_1$=$\beta_2$=$\beta_3$=1/3 and $\gamma_1$=$\gamma_2$=0.5, the $CF_t$ for each task are:
%\begingroup\makeatletter\def\f@size{8}\check@mathfonts
%\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
%\begin{align}
%	&\textit{CF_{T2}} = \beta_1 (\frac{0.8}{0.8}) + \beta_2(\frac{50\times 0.8}{50\times 0.8}) + \beta_3 (\frac{\gamma_1(100)+\gamma_2(1)}{\gamma_1(100)+\gamma_2(1)})=1 \nonumber \\
%	&\textit{CF_{T3}} = \beta_1 (\frac{0.6}{0.8}) + \beta_2(\frac{60\times 0.6}{50\times 0.8}) + \beta_3 (\frac{\gamma_1(100)+\gamma_2(1)}{\gamma_1(100)+\gamma_2(1)})=\frac{53}{60} \nonumber \\
%	&\textit{CF_{T4}} = \beta_1 (\frac{0.4}{0.8}) + \beta_2(\frac{90\times 0.4}{50\times 0.8}) + \beta_3 (\frac{\gamma_1(0)+\gamma_2(0)}{\gamma_1(100)+\gamma_2(1)})=\frac{11}{30} \nonumber 
%\end{align}	
%\begingroup\makeatletter\def\f@size{10}\check@mathfonts
%\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}
%Since the units of each item in the cost function are not the same, we normalize each item to bring all the values to the same range.
%So, $CF_{T2}$ > $CF_{T3}$ > $CF_{T4}$, which is reasonable due to the more energy and peak power consumption of task $T_2$ that should be mapped to the core with the lower $CF_c$. In addition, as can be computed, $CF_{C3}$~=~$CF_{C2}$~>~$CF_{C1}$.
So, $Eng_{T2}$ > $Eng_{T3}$ = $Eng_{T4}$ that shows $T_2$ should be mapped to the core with less accumulated energy ($E_c$). In addition, as can be computed, $E_{C3}$=$E_{C2}$>$E_{C1}$.
Therefore, according to the criticality level, we first map $T_2$ and $T_3$ on $C_3$ and $C_2$ and schedule them, and thereafter, $T_4$ is mapped on $C_4$. 
This procedure will be the same for mapping and scheduling $T_5$ and $T_6$.


It should be noted that the time complexity analysis and memory space analysis of the proposed method have been discussed in Appendix B and C of~\cite{Ranjbar2021}, respectively.


==> Sections/ResultsFinal.tex <==
\section{Experiment}
\label{sec:expriment}

%%In this section, we first introduce the experimental setups, and then evaluate the effectiveness of our proposed method and state-of-the-arts.

%In this section, we first introduce the experimental setups. We then evaluate the effectiveness of our proposed method in terms of schedulability, LC tasks' QoS, peak power management, and thermal distribution.

\subsection{Experimental Setup}
\label{subsec:experimentalSetup}

\subsubsection{Application}
\label{subsec:appsetup}

\behnaz{For the experiments, we used both real-life and random applications to show our proposed approach's efficiency. To generate random task graphs, we used the tool presented by Medina et al. \cite{Medina18}.}
We generated applications with 30, 40, 50, and 100 tasks (\textit{n}), where 20\% to 50\% of them are LC tasks.
Another important parameter in a task graph is edge percentage (\textit{d}) that shows the probability of having edges from one task to other tasks. We considered 1\% to 20 \% edge percentage in the experiments.
Another important parameter that will be discussed in the experiments is 
the normalized system utilization $U/c$, where $U$ is the utilization of the system considering the high WCET of each task, and $c$ is the number of cores.
\behnaz{We considered different values of normalized system utilization in the range of (0,1] with the steps of 0.05. We also evaluate the proposed approach and other approaches for comparison, with a real-life application task graph, vehicle cruise controller (CC)~\cite{izosimov10}, composed of 32 tasks, where 34\% of them are LC tasks. \answersnd{In addition, the value of edge percentage for this CC application is 7\%.}}




\subsubsection{Hardware Platform}
\label{subsec:archsetup}
\behnaz{To evaluate our approach, we conduct the experiments and run the applications on a platform with 2, 4, 8, and 16 cores, which models ARM Cortex-A7 cores~(\textit{c}).}
The maximum number of transient faults that may occur during each application period (\textit{k}) and the recovery overhead~$\mu$ are considered three and 15ms, respectively~\cite{Izosimov08}.
\behnaz{It is important to know that if $\lambda$ and $time$ is the fault rate and application execution time, respectively, the minimum number of fault occurrence would be $\lambda\times time$. Therefore, $k$ would not be much smaller or larger than $\lambda\times time$~\cite{Zhang2006}. If $\lambda=10^{-6}fault/\mu s$, and $time=10^{3}ms$, then, $\lambda\times time=1$. As a result, since this fault rate is much higher than real fault rates, mentioned $10^{-12}fault/\mu s$ in~\cite{Salehi2016}, considering $k\leq 3$ is reasonable fault occurrence number during each application period.}
We use the HOTSPOT tool~\cite{huang06} to obtain the cores' temperature trace by exploiting the specific floorplan according to a real platform, ODROID XU3 board, which has four ARM Cortex-A7 cores, and the parameters used in \cite{Gong2018}.
In addition, we use the reported value in \cite{Chisholm17}, to consider the timing overhead of mode switching for ARM Cortex processors. 
We considered the maximum reported overhead, which is $T_{sw}= 254 \mu s$, in our experiments.



\subsubsection{Peak Power Consumption}
\label{subsec:experimentalSetuppowe}

\answersnd{To determine a realistic power consumption for tasks, we ran several embedded benchmarks from the MiBench suite, such as automotive, network, and Telecomm., on ARM Cortex-A7 core of ODROID XU3 platform with maximum frequency at design-time. We monitor the power sensors continuously, and we set the worst measured power as the power consumption of tasks.}
In addition, we examined different scenarios of activating one core to all cores by running different benchmarks. 
Each benchmark is run 1000 times on a core, and we considered each task's power consumption between the minimum and maximum power values obtained from the platform. The measurement reports show that the power consumption of tasks is between 483\textit{mW} to 939\textit{mW}.
%Ali%It is noteworthy to mention that the power consumption of the system is the sum of the power consumption of all cores \cite{munawar14}. 
%\behnaz{Since the ODROID board has the power sensor for each cluster, which contains four homogeneous cores, the power sensor data shows the instantaneous power consumption of the cluster. }
%Ali%As mentioned before, the instantaneous power of a system should not be more than the TDP constraint. So, the power consumption of a system is computed periodically in a unit of time and compared to the TDP value. 
In this paper, the TDP value has been considered 85\% of the maximum power that a chip can consume, which is used conventionally in embedded processors \cite{liu07}.

\subsubsection{Comparison}
%\ali{
We analyzed our proposed method and compared our experimental results to the results obtained by recent works that use the task graph model~\cite{socci15,Medina18,Ranjbar19}. Socci et al. \cite{socci15} have proposed an online scheduling algorithm for an MC system where only HC tasks are executed in the HI mode. Medina et al. \cite{Medina18} has considered a fault-tolerant MC system that generates two tables at design-time and uses them at run-time (see \sectionRef{sec:relatedWork} for more details). Based on this work, researchers in~\cite{Ranjbar19} have presented an online approach to reduce the peak power and temperature by using the DVFS technique. Hence, due to the timing overhead of DVFS and increasing fault rate by changing the \textit{V-f} levels~\cite{koren07}, we cannot easily use this technique especially in the HI mode. 
%}


\subsection{Experimental Results}
\label{subsec:experimentalResults}



\subsubsection{\textbf{Tree Construction Time}}
At first, we evaluate offline tree construction time by varying the parameters $n$ and $k$, in \figureRef{fig: constructtime}. % and running 100 task sets for each point. 
The tree's construction time is computed on a system with an intel core-i5 processor with 1.3 GHz clock frequency. 
Construction time depends on the number of faults and tasks. \figureRef{VaryingTasksTime} shows the effects of the number of tasks and the portion of HC tasks in each task set with $k=3$. Besides, \figureRef{VaryingFaultTime} shows the effects of the number of fault occurrence with $n=20$. 
These figures depict that by increasing the number of faults or number of tasks, the tree generation's time is increased exponentially. Also, task sets with higher HC tasks have higher tree construction time. 
%\behnaz{According to our discussion in Section~\ref{subsubsec:treegenerate} and in the end, showing in Eq.~\ref{eq:treetimec}, the tree construction time has been grown exponentially by increasing the number of faults~($O(n^k)$, where \textit{n} and \textit{k} are the number of tasks and the number of faults, respectively and $n>>k$). }
Although the offline tree construction time is relatively high for large applications, the online overhead is small and constant for all applications. It is noticeable that our method can generate each node of a tree in parallel to reduce the construction time. For example, if we have a system with four cores, the construction time is about four times faster than a single-core system. 

\begin{figure}[t]
	\centering
	\begin{minipage}[t!]{1\linewidth}
		\centering
        \subfloat[Number of tasks]{\includegraphics[width=0.48\columnwidth]{imgs/TimeTask2.pdf}\label{VaryingTasksTime}}
        \hspace{4pt}
        \subfloat[Number of fault occurrence]{\includegraphics[width=0.48\columnwidth]{imgs/TimeFault2.pdf}\label{VaryingFaultTime}}
		\caption{Tree construction time for different application sizes and number of fault occurrence}
		\label{fig: constructtime}
	\end{minipage}
	%\includegraphics[width=0.83\columnwidth]{imgs/constime.pdf}
	%\caption{Tree construction time for different application sizes.}
	%\label{fig: constructtime}
\end{figure}

%Although the offline tree construction time is relatively high for large applications, the online overhead (it will be discussed in the next subsection) is very small and relatively constant for all applications. 
%It is noticeable that our method can generate each node of a tree in parallel to reduce the construction time. For example, if we have a system with four cores, it's about four times faster than constructing the tree with a single-core of the processor.
%The construction time of generating the tree in parallel on a system with an intel core-i7 processor is also presented in \figureRef{fig: constructtime}, which is about four times faster than constructing the tree with a single-core of the processor.

%\vspace{2pt}
\subsubsection{\textbf{Run-Time Timing Overheads}}


In case of fault occurrence or mode switching, the system finds the proper schedule by moving to the child of the current node, which is responsible for the upcoming scenario. 
Each node of the tree stores two arrays with the size of $n\times (log^{c}_2+log^{\frac{period}{timeslot}}_2)$ bits, where $c$ and $n$ are the number cores and tasks, respectively.
Thus, the switching time between the schedules consists of moving one level in the tree and retrieving the correct scheduling from memory, which is constant and negligible.
We measured the schedule changing time at run-time on the ODROID XU3 platform, considering $c=8$, and $n=50$, it is almost 0.47$\mu$s.

%just the required time to decode from memory. If we consider the ODROID XU3 platform, the decoding time is 140 $MB/s$. For example, if we consider $c=8$, and $n=50$ with the period of 1000$ms$ for a graph, we store 520 $bits$ (65byte) for two arrays. Therefore, the decoding time is almost 0.47$\mu$s (i.e., in the range of nanosecond) and can be negligible.
%

%To search within a tree structure and find the proper schedule, since we are in a certain path and the current node of the tree is known, the system just checks the current node's successors to select the desired one. Therefore, if it has $r$ successors, the time complexity is $O(r)$, and its consuming time is in the range of nanosecond and negligible.
%
%%Switch between schedules
%%As mentioned in Section~\ref{subsec:Memory Space Overhead}, 
%We store two arrays for each schedule with the size of the number of tasks that need $n\times (log^{m}_2+log^{\frac{period}{timeslot}}_2)$ bits, where $m$ and $n$ are the number cores and tasks, respectively. 
%Therefore, if a schedule is changed during runtime, just the new arrays are decoded from memory to exploit and read each task's data. Thus, the switching time between the schedules is just the required time to decode from memory. If we consider the ODROID XU3 platform, the decoding time is 140 $MB/s$. For example, if we consider $c=8$, and $n=50$ with the period of 1000$ms$ for a graph, we store 520 $bits$ (65byte) for two arrays. Therefore, the decoding time is almost 0.47$\mu$s (i.e., in the range of nanosecond) and can be negligible.


%\vspace{2pt}
\subsubsection{\textbf{Peak Power Management and Thermal Distribution for a Real-Life Application}}
\label{subsec:CCPowTempTrace}

\behnaz{\figureRef{fig: PowerCC} shows the system's power traces of a real-life application, vehicle Cruise Controller (CC)~\cite{izosimov10} by our proposed approach, the approaches proposed by Socci et al.~\cite{socci15}, Medina et al.~\cite{Medina18}, and Ranjbar et al.~\cite{Ranjbar19}. Since~\cite{Ranjbar19} is the online approach to minimize the peak power, while exploiting the same task mapping and scheduling of~\cite{Medina18} at design-time, their power traces and thermal distributions are the same in the worst-case scenario of tasks' execution time and power consumption. %This section shows the real application results, and we show the results of runnig a random task graph example in Appendix~B. 
}%~\ref{A-ExpPowTemp}.}
In this part, to focus on the behavior of systems in the HI mode, we assumed no fault occurred during the application's execution.
Socci's approach does not violate TDP constraint because it drops all LC-tasks when the system switches to the HI mode, which means it has zero-percent QoS of LC tasks in the HI mode.
On the other hand, methods of~\cite{Medina18} and~\cite{Ranjbar19} guarantee 90.91\% of LC tasks execution in the HI mode, but it frequently violates the TDP constraint (\figureRef{fig: PowerCC}).
For the CC application, our method endeavored to execute 81.82\% of the LC tasks without violating TDP constraint. 
Appendix~D of~\cite{Ranjbar2021} shows the thermal distribution of CC application and also, the corresponding results for a random task set with high utilization.

%\begin{figure}[t]
%	\centering
%    \begin{minipage}{1\linewidth}
%		\centering
%		\includegraphics[width=0.84\textwidth]{imgs/CCPowernew2.pdf}
%		\caption{Power trace of real-life application graph (CC) using different methods.}
%	    \label{fig: PowerCC}
%	\end{minipage}
%%\vspace{-20pt}	
%\end{figure}
%\figureRef{fig:realLifeScenarios} shows the steady-state temperature distribution of Sooci~\cite{socci15}, Medina~\cite{Medina18}, Ranjbar~\cite{Ranjbar19}, and our proposed method using the HOTSPOT simulator. Although the maximum temperature of~\cite{socci15} is lower than ours, it has zero-percent LC tasks' QoS because it does not execute any LC task in the HI mode. In addition, we map the tasks on the cores more uniform than the Medina's method, which prevents hotspots in our approach. \behnaz{The proposed approach could reduce 5$^\circ$C in maximum temperature compared to~\cite{Medina18,Ranjbar19}. If the system becomes larger in terms of number of cores and tasks, the efficiency of our proposed approach in reducing the hotspots would be higher. Appendix~D shows the corresponding results for a random task set with high utilization. }

\behnaz{As a result, our method reduces the peak power and maximum temperature by up to 20.06\% and 3.71\% respectively, compared to the approach of~\cite{Medina18,Ranjbar19}, while the QoS is degraded 9.09\%. On the other hand, although our method increases the maximum temperature by 9.61\%, compared to~\cite{socci15}, we reduce the peak power consumption by 6.31\% and improve the QoS by 81.82\%.}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.765\columnwidth]{imgs/CCPowernew4.pdf}
	\caption{Power trace of real-life application graph (CC) in different methods under worst-case scenario}
	\label{fig: PowerCC}
\end{figure}



% \begin{figure}[t]
% 	\begin{minipage}[t]{1\linewidth}
% 		\centering
% 		%\includegraphics[width=\textwidth]{imgs/localsystem.pdf}
% 		\subfloat[Proposed Method]{\includegraphics[width=0.28\textwidth]{imgs/CCOurs.pdf}\label{fig:fig11a}}
%         \hfil
%         \subfloat[\cite{Medina18,Ranjbar19}]{\includegraphics[width=0.28\textwidth]{imgs/CCMedina.pdf}\label{fig:fig11b}}
%         \hfil
%         \subfloat[\cite{socci15}]{\includegraphics[width=0.28\textwidth]{imgs/CCHI.pdf}\label{fig:fig11c}}
%         \hfil
%         \subfloat{\includegraphics[width=0.07\textwidth]{imgs/CCBarnew1.pdf}\label{fig:fig11d}}
% 		\caption{Thermal profiles of real-life application graph (CC) in different methods under worst-case scenario.}
%         \label{fig:realLifeScenarios}
% 	\end{minipage}
% \end{figure}






%\vspace{2pt}

%\vspace{2pt}
\subsubsection{\textbf{Analyzing the QoS of LC Tasks}}
\label{subsec:QoSAnalysis}

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{imgs/QoSAnalysis6-1.pdf}
	\caption{Task sets' QoS under different scenarios}
	\label{LCTQoS}
\end{figure}

\begin{figure*}[t!]
	\centering
	\begin{minipage}[t!]{1\linewidth}
		\centering
        \subfloat[Varying Utilization]{\includegraphics[width=0.25\columnwidth]{imgs/PTVu1.pdf}\label{PTVaryingUtil}}
        \hfil
        \subfloat[Varying Number of Tasks]{\includegraphics[width=0.23\columnwidth]{imgs/PTVn1.pdf}\label{PTVaryingTasks}}
        \hfil
        \subfloat[Varying Edge Percentage]{\includegraphics[width=0.23\columnwidth]{imgs/PTVd2.pdf}\label{PTVaryingEdge}}
        \hfil
        \subfloat[Varying Number of Cores]{\includegraphics[width=0.25\columnwidth]{imgs/PTVc2.pdf}\label{PTVaryingCores}}
		\caption{Peak power consumption and maximum temperature in different methods}
		\label{PPowerResult}
	\end{minipage}
\end{figure*}


\behnaz{Now, we analyze the QoS for the proposed method in comparison with methods of~\cite{socci15,Medina18,Ranjbar19} in~\figureRef{LCTQoS}.} %shows the LC tasks' QoS analysis for the proposed method in comparison with methods of~\cite{socci15,Medina18,Ranjbar19}}.
In our proposed method, there are many possible scenarios (each node of the tree is responsible for keeping the scheduling of system in one scenario), and for each scenario, the LC tasks' QoS is different. 
Thus, we run 100 schedulable task sets on eight cores, and for each task set, 10 different random situations of occurring faults and mode switching are considered. For the case when $U/c$=[0.5,0.75) or $U/c$=[0,0.5), there is more free slack before task set deadline; therefore, in the case of fault occurrence and mode switching, fewer LC tasks are dropped. 
In this experiment, we consider the worst-case scenario of processor demands, $U/c$= [0.75,1], $n$= 50 and $d$=10\% and in the generated task sets, 20\% to 50\% of tasks are LC tasks. In addition, the number of fault occurrences in each scenario is randomly selected in the range of [0,4]. \figureRef{LCTQoS} shows the LC tasks' QoS for all these 1000 scenarios. 
\behnaz{In Section~\ref{subsec:mixedCriticalityTaskModel}, we have defined the QoS as the successfully executed LC tasks to all LC tasks. However, we use three different definitions of QoS to evaluate the methods of~\cite{Medina18,Ranjbar19,socci15} more accurately, as follows. 
\begin{itemize}[leftmargin=*]
    \item Scenario~1: The QoS refers to How many LC tasks are successfully executed before their deadlines with no TDP violation. If TDP is going to be violated, running LC tasks are only stopped to reduce the peak power consumption.
    \item Scenario~2: This scenario has the same definition as Scenario~1, with the difference that since the HC tasks are the most important, therefore without them, QoS of LC tasks is penalized by completely being zero. Thus, if TDP is violated and some HC tasks are running on cores, then the QoS=0. 
    \item Scenario~3: Since those methods have not been specifically designed for peak power management while meeting the real-time constraints of all HC tasks, we give the HC tasks higher weighted and then consider the joint QoS, including both LC and HC tasks. Therefore, the HC tasks have a double weight in this scenario compared to LC tasks, in the case of dropping tasks due to the TDP violation.
\end{itemize}}

\behnaz{As shown in~\figureRef{LCTQoS}, the QoS for methods of~\cite{Medina18,Ranjbar19} in Scenario~1 is higher than the QoS for our proposed method in total (according to the Cumulative Distribution Function (CDF) line). However, in this scenario, the TDP constraint is violated several times due to the execution of HC tasks in parallel on cores, and there is no policy to manage the peak power. Moreover, for the second scenario in the methods of~\cite{Medina18,Ranjbar19}, the figure shows that in 22.5\% of task sets, the TDP constraint is violated while executing some HC tasks on cores. Besides, the QoS in the second scenario for~\cite{socci15} is zero, due to dropping all LC tasks in the HI mode. Now, if we investigate the methods of~\cite{Medina18,Ranjbar19,socci15} in the third scenario, the QoS of~\cite{Medina18,Ranjbar19} is more than the QoS of~\cite{socci15} due to the executing LC tasks in the HI mode. However, they have less QoS in this scenario compared to our proposed method. 
According to this figure, we can conclude that our proposed method is more efficient in improving QoS than other methods in different scenarios.} In addition, the minimum and maximum QoS in our proposed method are 68.33\% and 100\%, while the power constraint is always met.%, and 44.7\% of the task sets have the maximum value of QoS. }
%According to our proposed method in Section~\ref{subsec:treeConstructionStrategies}, we drop a LC task with the largest execution time in the HI mode to improve the QoS. If this policy is not used, the average QoS is 88.70\%. (4.4\% degradation).



%\vspace{2pt}

\subsubsection{\textbf{Peak Power Consumption and Maximum Temperature Analysis}}
\label{subsec:PowTempAnalysis}

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.99\columnwidth]{imgs/TDP1.pdf}
%	\caption{Peak power consumption and max. temperature in different methods.}
%	\label{PPowerResult}
%\end{figure}




%In this section, we evaluate the system's peak power consumption in our approach and Medina's method~\cite{Medina18} with different parameters. Fig.~\ref{PPowerResult} shows the average normalized peak power consumption to the TDP constraint in the worst case that the system switches to the HI mode after executing the first HC task and all tasks execute up to their WCET. The figure shows that our proposed approach's peak power consumption is less than the TDP constraint in all scenarios, while Medina's method violates the TDP constraint almost all scenarios. \behnaz{In general, the impact of our approach increases as the probability of using parallelism in the execution of tasks on cores increases (a large number of cores (larger \textit{c}) or less dependency between tasks (lower \textit{d})). Since the number of tasks and utilization are not changed by increasing \textit{c}, the maximum power consumption by~\cite{Medina18} is also reduced. However, since our proposed method endeavors to distribute the tasks on all cores to reduce hotspots and also minimize the instantaneous power consumption, the efficiency of our proposed approach in decreasing the peak power consumption is more, compared to~\cite{Medina18}, while the \textit{c} is increased. Besides, with decreasing the dependency between tasks (\textit{d}), although the system peak power consumption is increased and TDP is violated in~\cite{Medina18}, our approach always guarantees that the TDP constraint is not violated.}
%The impact of our approach increases as the probability of using parallelism in the execution of tasks on cores increases (a large number of cores (larger \textit{c}) or less dependency between tasks (lower \textit{d})). In addition, although increasing the number of tasks (\textit{n}) or utilization increases the system's peak power consumption because the system does more computation, our approach guarantees that the TDP constraint will never be violated.

In this section, we evaluate the system's peak power consumption and the chip's maximum temperature in our approach and methods of~\cite{Medina18,Ranjbar19} by varying different parameters, such as utilization bound ($U/c$), number of tasks ($n$), edge percentage ($d$), and the number of cores ($c$). Fig.~\ref{PPowerResult} shows the average normalized peak power consumption to the TDP constraint and maximum temperature in the worst case that the system switches to the HI mode after executing the first HC task and all tasks execute up to their higher WCET. Hence, in the worst-case scenario, \cite{Ranjbar19} has the same power profile and thermal distribution as~\cite{Medina18}.

First, we analyze the peak power consumption by varying different parameters. The figure shows that our proposed approach can manage the peak power consumption to be less than the TDP constraint in all scenarios, while Medina's method violates the TDP constraint almost all scenarios. 
\behnaz{In general, the impact of our approach is increased as the probability of using parallelism in the execution of tasks on cores is increaseed (a large number of cores (larger \textit{c}) or less dependency between tasks (lower \textit{d})). 
Since the number of tasks and utilization are not changed by increasing \textit{c}, the maximum power consumption by~\cite{Medina18} is also reduced. However, since our proposed method endeavors to distribute the tasks on all cores to minimize hotspots and also minimize the instantaneous power consumption, our proposed approach in decreasing the peak power consumption is more efficient, compared to~\cite{Medina18}, while the \textit{c} is increased. Besides, by reducing the dependency between tasks (\textit{d}), although the system peak power consumption is increased and TDP is violated in~\cite{Medina18}, our approach always guarantees that the TDP constraint is not violated.}
%The impact of our approach increases as the probability of using parallelism in the execution of tasks on cores increases (a large number of cores (larger \textit{c}) or less dependency between tasks (lower \textit{d})). 
In addition, although increasing the number of tasks or utilization increases the system's peak power consumption because the system does more computation, our approach guarantees that the TDP constraint will never be violated.


From the perspective of maximum temperature analysis, increasing the system utilization, illustrated in Fig.~\ref{PTVaryingUtil}, while the number of tasks is fixed ($n$=~50) means that the task's execution time tends to be longer. Thus, the computation time of cores is increased, the managing of peak power constraint and busy/idle times of cores would be difficult, and consequently, the maximum temperature of the chip is increased in both methods. However, \behnaz{we can decrease the maximum temperature by up to % 19.65\% 
22.4$^\circ$C in comparison with~\cite{Medina18,Ranjbar19}. Besides, if we vary the number of tasks in Fig.~\ref{PTVaryingTasks}, since the computation time of cores does not change, the chip's maximum temperature is relatively constant by increasing the number of tasks in both our proposed method and methods of~\cite{Medina18,Ranjbar19}.} Additionally, by varying~\textit{d}, the maximum temperature reduces by increasing the dependency between tasks because the cores' computation time is constant, while the idle time of cores is increased. \behnaz{As shown in Fig.~\ref{PTVaryingEdge}, our proposed method can reduce the maximum temperature by %14.64\%
14.3$^\circ$C on average by varying edge percentage, compared to~\cite{Medina18,Ranjbar19}.}

\begin{figure*}[t!]
	\centering
	\begin{minipage}[t!]{1\linewidth}
		\centering
        \subfloat[Varying Utilization]{\includegraphics[width=0.24\columnwidth]{imgs/utilsch2.pdf}\label{VaryingUtil}}
        \hfil
        \subfloat[Varying Number of Tasks]{\includegraphics[width=0.23\columnwidth]{imgs/tasksch2.pdf}\label{VaryingTasks}}
        \hfil
        \subfloat[Varying Edge Percentage]{\includegraphics[width=0.23\columnwidth]{imgs/edgesch2.pdf}\label{VaryingEdge}}
        \hfil
        \subfloat[Varying Number of Cores]{\includegraphics[width=0.23\columnwidth]{imgs/coresch3.pdf}\label{VaryingCores}}
		\caption{Normalized acceptance ratio under different scenarios in different methods}
		\label{Varying}
	\end{minipage}
\end{figure*}



Now, we investigate the system's maximum temperature in Fig.~\ref{PTVaryingCores} by increasing the number of cores (\textit{c}) while other parameters are constant. Hence, the normalized utilization (\textit{U/c} is constant in this experiment, it means the utilization (U) is increased by increasing \textit{c}. We have more parallelism to execute tasks by increasing \textit{c} and add more free slack to let the cores be idle (having better thermal distribution). However, since each core's temperature is a function of its neighbor cores' temperature, it increases the chip's maximum temperature while the system utilization is increased. \behnaz{Therefore, the results of our proposed method show that the maximum temperature is relatively constant by increasing \textit{c} and can decrease it, %11\% (
10.7$^\circ$C on average, compared to~\cite{Medina18,Ranjbar19}. Since the methods of~\cite{Medina18,Ranjbar19} do not consider the thermal distribution, the maximum temperature is generally increased by increasing~\textit{c}.}


%\vspace{2pt}
%\subsubsection{\textbf{Effect of \textit{d}, \textit{n}, \textit{U}, and \textit{c} Parameters on Schedulability and Max. Temperature}}
%\subsubsection{\textbf{Effect of Varying \textit{d}, \textit{n}, \textit{U}, and \textit{c} Parameters on Acceptance Ratio}}
\subsubsection{\textbf{Effect of Varying Different Parameters on Acceptance Ratio}}
\label{subsec:SchAnalysis}
%In this section, we illustrate the impact of different parameters, such as utilization bound ($U/c$), number of tasks ($n$), edge percentage ($d$), and the number of cores ($c$) on the task schedulability and the chip's maximum temperature. \figureRef{Varying} represents the effect of each parameter, while the others are fixed, to analyze how the proposed method reacts to each parameter. \behnaz{In this section, we run 1000 benchmarks for each scenario which are schedulable by the Medina's approach~\cite{Medina18} and report the average result (that are normalized to the approach of~\cite{Medina18}) to show the efficiency of our proposed method.} In general, having more dependency between tasks, large system utilization, or more cores, causes the system to have less task schedulability.

In this section, we illustrate the impact of different parameters, such as utilization bound ($U/c$), number of tasks ($n$), edge percentage ($d$), and the number of cores ($c$) on~the task schedulability (acceptance ratio). 
\behnaz{\figureRef{Varying} represents the effect of each parameter, while the others are fixed, to analyze how the proposed method and the methods of~\cite{Medina18,Ranjbar19} react to each parameter. 
%In this section, 
We run 1000 benchmarks for each scenario, % that are schedulable in term of real-time constraint by the Medina's approach~\cite{Medina18}
and report the average result. A task set is schedulable if the real-time and power constraints are met.% (that are normalized to the approach of~\cite{Medina18}) to show the efficiency of our proposed method.
} 
In general, having more dependency between tasks, large system utilization, or more cores, causes the system to have less acceptance ratio in our proposed method. We discuss the observation in detail.


From the perspective of utilization bound, we fix other parameters to see the effective of varying utilization in~\figureRef{VaryingUtil}. Increasing the utilization while the number of tasks is fixed ($n$=~50), means that the tasks execution time tends to be longer. when the utilization is getting higher, the computation time of cores is increased. Therefore, fewer task sets can be scheduled before their deadlines even in the case of fault occurrence, and also, the managing of power constraint and busy/idle times of cores would be difficult. %, and consequently, the maximum temperature of the chip is increased. 
We can conclude that fewer task sets can be scheduled before their deadline, while the power constraint is not violated. \behnaz{This trend is also the same with~\cite{Medina18,Ranjbar19} with the difference that the TDP constraint is violated several times, which causes the task sets not to be schedulable.}% In addition, the task migration has been used several times to manage the real-time constraints in~\cite{Medina18}, %they can well map and schedule tasks 
%for the high system utilization. However, the authors have not considered the migration timing overhead, which may cause serious deadline violations. }

Besides, \figureRef{VaryingTasks} shows that the task schedulability is increased by increasing the number of tasks, with $d$=~10\%, $U/c$=~[0.5,0.75), and $c$=~8. Since the system utilization is constant for all number of tasks, the execution time of tasks is reduced by increasing the number of tasks. Therefore, the tasks tend to finish their execution early and allow their successors to be released. Furthermore, the overhead of re-executing a task due to fault occurrence is much lower for small tasks.
According to~\figureRef{VaryingTasks}, we conclude that our method can schedule \behnaz{70\%} of task sets, on average, when only the number of tasks is varied. %and other parameters are fixed. 
\behnaz{Besides, by increasing the number of tasks in the methods of~\cite{Medina18,Ranjbar19}, %have used the migration policy during the execution of tasks to meet their deadlines (but without considering the migration timing overhead), they can schedule more task sets while the number of tasks is less.
the parallel task execution is increased, which causes more peak power consumption, and therefore, less task schedulability due to the TDP violation. }%However, by increasing the number of tasks, the peak power consumption tends }%From the maximum temperature perspective, since the computation time of cores does not change, the chip's maximum temperature is relatively constant by increasing the number of tasks.


% Version2
% \begin{figure}[t!]
% 	\centering
% 	\begin{minipage}[t!]{1\linewidth}
% 		\centering
%         \subfloat[Utilization]{\includegraphics[width=0.305\columnwidth]{imgs/utilsch1.pdf}\label{VaryingTasks}}
%         \hfil
%         \subfloat[Number\\ of Tasks]{\includegraphics[width=0.25\columnwidth]{imgs/tasksch.pdf}\label{VaryingUtil}}
%         \hfil
%         \subfloat[Edge\\ Percentage]{\includegraphics[width=0.2\columnwidth]{imgs/edgesch.pdf}\label{VaryingEdge}}
%         \hfil
%         \subfloat[Number\\ of Cores]{\includegraphics[width=0.225\columnwidth]{imgs/coresch.pdf}\label{VaryingCores}}
% 		\caption{Normalized acceptance ratio under different scenarios.}
% 		\label{Varying}
% 	\end{minipage}
% \end{figure}

%\begin{figure*}[t!]
%	\centering
%	\begin{minipage}[t!]{1\linewidth}
%		\centering
%        \subfloat[Varying Number of Tasks]{\includegraphics[width=0.24\columnwidth]{imgs/FigTT2.pdf}\label{VaryingTasks}}
%        \hfil
%        \subfloat[Varying Utilization Bound]{\includegraphics[width=0.24\columnwidth]{imgs/FigUT2.pdf}\label{VaryingUtil}}
%        \hfil
%        \subfloat[Varying Edge Percentage]{\includegraphics[width=0.24\columnwidth]{imgs/FigET2.pdf}\label{VaryingEdge}}
%        \hfil
%        \subfloat[Varying Number of Cores]{\includegraphics[width=0.24\columnwidth]{imgs/FigCT2.pdf}\label{VaryingCores}}
%		\caption{Task schedulability percent and maximum temperature under different scenarios.}
%		\label{Varying}
%	\end{minipage}
%\end{figure*}





For the case of varying the edge percentage, when the dependency between the tasks is increased, while $n$, $U/c$ and $c$ are constant ($n$=~50, $U/c$=~[0.5,0.75), $c$=~8), the release time of tasks is increased, because tasks must wait for more predecessor tasks to finish their executions. 
Therefore, the idle time on cores increases, which causes more delays in the execution of tasks, and reduce the schedulability. 
\figureRef{VaryingEdge} shows that the highest schedulability (73\%) is achieved in our method when $d$=1\%. 
%Besides, \figureRef{VaryingEdge} shows that the maximum temperature reduces by increasing the dependency between tasks because the cores' computation time is constant, while the idle time of cores is increased.
\figureRef{VaryingCores} shows the effect of varying the number of cores in the system on task schedulability when other parameters are not changed ($n$=~50, $U/c$=~[0.5,0.75), $d$=~10\%). 
By considering the fixed $U/c$, the utilization is increased by increasing the number of cores.
Consequently, the execution time of tasks is increased  %when the system utilization is increased 
because the number of tasks is fixed. 
As mentioned earlier, the task schedulability is decreased by increasing the tasks' execution time. Therefore, as can be seen in~\figureRef{VaryingCores}, the schedulability of applications with our proposed method decreases by increasing the number of cores, while the other parameters are fixed. 
Besides, in methods of~\cite{Medina18,Ranjbar19}, the acceptance ratio increases by increasing the dependency between tasks and having more cores in the system. The reason is that based on their mapping and scheduling algorithm, \answersnd{by increasing the edge percentage and number of cores while fixing other parameters, tasks have less parallelism, and also fewer cores are selected to be active to execute the tasks, which causes the system to have less peak power consumption and therefore, a higher acceptance ratio. As a result, by increasing the edge percentage for more than 20\%, our proposed method and method of~\cite{Medina18,Ranjbar19} have almost the same acceptance ratio.} However, the mapping and scheduling algorithm of~\cite{Medina18,Ranjbar19} increases the overheating problem, which is not acceptable by most safety-critical systems. % and sometimes is less than TDP constraints. 
In addition, since methods of~\cite{Medina18,Ranjbar19} are not peak-power aware, %task mapping and scheduling, 
when the number of cores is less, the TDP is violated in most of the task sets and therefore, these task sets are not schedulable.
%Besides, if we investigate the system's maximum temperature, by increasing the number of cores, we have more parallelism to execute tasks and add more free slack to let the cores be idle. However, since each core's temperature is a function of the temperature of its neighbor cores, it increases the chip's maximum temperature. However, the results show that the maximum temperature is relatively constant by increasing the number of cores.

\behnaz{In the end, the acceptance ratio of our proposed method is 74.14\% on average for all scenarios, while it is 31.1\% in the methods of~\cite{Medina18,Ranjbar19}.}% Therefore, we can claim that we have a 13.09\% improvement in comparison with~\cite{Medina18,Ranjbar19}.}


\subsubsection{\textbf{\behnaz{Investigating Different Approaches at Run-Time}}}%, in Terms of Peak Power Consumption}}
\label{subsec:RuntimePowTrace}


\behnaz{Now, we evaluate the system behavior at run-time in terms of peak power consumption for our proposed approach and the method proposed in~\cite{Ranjbar19,socci15,Medina18}.} Researchers in~\cite{Ranjbar19} have presented a run-time method to reclaim the available slacks and reduce the \textit{V-f} levels of cores to decrease the system peak power. Here, analogous to~\cite{Ranjbar19}, the actual execution time of tasks follows the normal distribution with the mean and standard deviation of $\frac{3\times WCET}{4}$ and $\frac{WCET}{12}$, respectively. Fig.~\ref{Runtimepowertrace} depicts the run-time power trace of methods for a random task graph with $d=10\%$, $n=50$, $c=8$ and $U/c=0.9$. The system switches to the HI mode by forcing a randomly selected HC task to execute beyond its lowest WCET for both methods. \behnaz{As shown in this figure, the system peak power in the proposed approach is less than the TDP constraint at run-time, while the method of~\cite{Medina18} has violated the TDP for a period of time. Although the system peak power of~\cite{Ranjbar19} may be less than the TDP constraint for some applications like the used task graph and their method consumes less energy in the system, there is no guarantee for the peak power to be less than the power constraint. Due to the using of DVFS technique in~\cite{Ranjbar19} and decreasing the \textit{V-f} levels at run-time, the system consumes less energy in comparison with our proposed method. For the example of Fig.~\ref{Runtimepowertrace}, the method of~\cite{Ranjbar19} saves 0.74102$J$ in system compared to our proposed approach.}
However, the DVFS technique degrades the reliability and increases the fault rate. The fault rate depends on the system's voltage level, and also, the application's reliability depends on the voltage level and tasks' WCET, which is increased by reducing the frequency level~\cite{Salehi2016}. 
As an example, for this task graph, by considering the fault rate $f=10^{-4}$~\cite{salehi16}, the reliability of tasks has been decreased $0.17\%$ and $2.08\%$, on average and worst-case in comparison with our proposed approach. In addition, the number of nines for the system's reliability ($-Log_{10}^{1-Rel}$) has been degraded from 8 to 6, which may not be desirable for most safety-critical applications~\cite{Ranjbar2020Fantom}.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.95\columnwidth]{imgs/onlinepow4.pdf}
	\caption{System power trace of different methods at run-time}
	\label{Runtimepowertrace}
\end{figure}


From the perspective of system's reliability and fault-tolerance in our proposed method, we run the 1000 task graph applications for different normalized utilization bound ($U/c$= [0.5,0.75), and [0.75,1]) and compare to the system's reliability in~\cite{Ranjbar19}. In our proposed method, $-Log_{10}^{1-Rel}$ for the normalized utilization equal to [0.5,0.75), and [0.75,1], is 8.56 and 7.67 on average, respectively, while for ~\cite{Ranjbar19}, is 4.99, and 4.60, respectively. 
As a result, based on the required reliability for safety-critical systems, the method of~\cite{Ranjbar19}, which decreases the \textit{V-f} levels, has severely damaged the system's safety, which is not desirable. The reliability of the proposed approach is high for different utilization. Therefore, our method can be applied to any application with varying bounds of utilization while satisfying the peak power management, fault-tolerance, and high reliability in different system operational modes. 
%The reliability of the proposed method is decreased by increasing the utilization bound. This is because there are more tasks in the system when utilization is increased. Therefore, finding the appropriate mapping and scheduling for tasks, while prevent the simultaneous execution of tasks on cores to manage the peak power, becomes complicated. Besides, the 


\behnaz{Besides, we have evaluated the proposed method and compared with the other methods at run-time by using the real task graph in Appendix E of~\cite{Ranjbar2021}.}



